SuperMemory-VQA: An Egocentric Visual Question-Answering Benchmark for Long-Horizon Memory

AI glasses present a compelling platform for AI agents to serve as personalized memory assistants. To be genuinely useful, such systems must move beyond short-term video comprehension and address memory gaps that humans experience for practical, personal, or social purposes over longitudinal egocentric video streams. However, existing egocentric datasets predominantly focus on action recognition or generic QAs from short clips, measuring perceptual capabilities rather than realistic human memory needs. We introduce SuperMemory-VQA, an egocentric visual question answering (VQA) dataset for evaluating AI assistants on practical, long-horizon memory tasks. It contains 52.9 hours of everyday activities recorded with AI glasses, including synchronized RGB video, audio transcription, eye gaze, IMU, and SLAM trajectories. Through a human-verified annotation pipeline, we construct grounded 4,853 question-answer pairs that span object and location memory, intent recall, visual scene recall, timeline reconstruction, conversational memory, and in-context retrieval. Each question is posed as multiple-choice with an explicit "unanswerable" option to test hallucination robustness. Benchmarking leading agentic frameworks and LLM backbones reveals that existing systems remain far from reliable on real-world memory tasks, highlighting the need for new architectures for grounded AI memory that can answer only when evidence is sufficient. A participant survey further supports that our questions are realistic, useful, and aligned with everyday memory needs.

==> sections/limitations.tex <==
\section{Limitations}
\label{app:limitations}
\label{sec:limitations}

\datasetName is an initial benchmark for long-horizon egocentric memory rather than an exhaustive representation of all daily-life settings. The current release contains \datasetHours hours of recordings from \numberOfParticipants participants, which is large enough to expose important retrieval, grounding, and answerability failures but still limited relative to the diversity of homes, cultures, languages, activities, and accessibility needs that future AR memory assistants will encounter. The dataset also relies on loosely scripted indoor and outdoor activities centered around a simulated home setting, so it may not capture the full unpredictability, privacy sensitivity, and behavioral diversity of unconstrained daily life.

At the same time, the benchmark is designed as a building block. The annotation pipeline separates dense captioning, structured ledger construction, agentic QA generation, verification, and human review. This modular design can be reused for future data collection efforts and scaled to additional participants, longer recordings, new environments, and specialized use cases. We view \datasetName as a foundation for measuring current system failures and for guiding larger future benchmarks for grounded AR memory with explicit evidence-sufficiency checks.

